Reasoning without Regret

Chain-of-thought reasoning enables large language models to solve multi-step tasks by framing problem solving as sequential decision problems. Outcome-based rewards, which provide feedback only on final answers, show impressive success, but face challenges with credit assignment and slow convergence. In contrast, procedure-based rewards offer efficient step-level feedback, but typically require costly human supervision. We introduce \emph{Backwards Adaptive Reward Shaping} (BARS), a no-regret framework that converts sparse outcomes-based rewards into effective procedure-based signals. BARS uses sparse rewards generated from terminal-state priors and cover trees to scale rewards while preventing exploitation. With Bellman contraction and $(\Delta, \epsilon)$-gap rewards, our backward Euler solver achieves $\epsilon$-accuracy in $O\left((R_{\max}/\Delta)\log(1/\epsilon)\right)$ iterations with $O(\log T)$ dynamic regret over $T$ rounds. Our analysis, based on generic chaining, continuous scaling limits, and non-linear Feynman-Kac bounds, connects recent outcome-based methods' empirical successes with the benefits of intermediate supervision. Combined, this provides the first rigorous no-regret algorithm for outcome reward shaping, providing a theoretical foundation for the empirical success of DeepSeek's R1.

==> reward-picture.tex <==
\begin{tikzpicture}[scale=1.5]

    % Define colors
    \definecolor{darkblue}{RGB}{0,0,150}
    \definecolor{brightblue}{RGB}{0,80,255}
    \definecolor{brightpurple}{RGB}{180,0,180}
    \definecolor{brightorange}{RGB}{255,120,0}
    \definecolor{brightorange}{RGB}{255,140,0}
    \definecolor{rewardcolor}{RGB}{255,140,0}
    \definecolor{brightolive}{RGB}{57,255,20}
    
  % Define gradient colors
  \definecolor{lowcolor}{RGB}{240,240,240}
  \definecolor{highcolor}{RGB}{70,130,180}
  
  % Define the non-convex shape with a smooth boundary
  \def\nonconvexshape{
    % Main blob shape
    (0,0) .. controls (1.5,0.5) and (2.5,-0.5) .. 
    (3,1) .. controls (3.5,2.5) and (2,3) .. 
    (1,2.5) .. controls (0.5,2.7) and (-0.5,2.2) .. 
    (-1,1.5) .. controls (-1.2,0.5) and (-0.8,-0.5) .. 
    (0,0) -- cycle
  }
  
  % Define reward points (sparse non-zero function values on/near boundary)
  \coordinate (R1) at (2.9,1.1);  % Reward point 1
  \coordinate (R2) at (-0.9,1.4); % Reward point 2
  \coordinate (R3) at (1.1,2.4);  % Reward point 3
  \coordinate (R4) at (0.1,-0.05); % Reward point 4
  
  % Define center point P_0
  \coordinate (P0) at (1.0,1.2);
  
  % Draw the base shape with gradient coloring
  \fill[lowcolor] \nonconvexshape;
  
  % Create radial fading gradients from each reward point
  \begin{scope}
    \clip \nonconvexshape;
    \foreach \point/\rad/\opac in {
      R1/1.2/0.8,
      R2/1.0/0.7,
      R3/1.1/0.9,
      R4/0.9/0.6
    } {
      \shade[inner color=highcolor, outer color=lowcolor, opacity=\opac] 
        (\point) circle (\rad);
    }
  \end{scope}
  
  % Draw the shape outline
  \draw[thick] \nonconvexshape;
  
  % Draw the forward paths (solid with arrows)
  % Continuous versions
  \draw[->, very thick, brightblue] (P0) .. controls (1.8,1.0) and (2.6,0.8) .. (R1);
  \draw[->, very thick, brightblue] (P0) .. controls (0.3,0.8) and (-0.5,0.9) .. (R2);
  \draw[->, very thick, brightblue] (P0) .. controls (0.8,1.8) and (0.9,2.2) .. (R3);
  \draw[->, very thick, brightblue] (P0) .. controls (0.8,0.6) and (0.5,0.1) .. (R4);
  
  % Extract the coordinates along the continuous forward paths
  % For R1 path
  \def\FOnePathXA{1.0}  \def\FOnePathYA{1.2}   % P0
  \def\FOnePathXB{1.3}  \def\FOnePathYB{1.15}
  \def\FOnePathXC{1.8}  \def\FOnePathYC{1.0}
  \def\FOnePathXD{2.2}  \def\FOnePathYD{0.9}
  \def\FOnePathXE{2.6}  \def\FOnePathYE{0.8}
  \def\FOnePathXF{2.9}  \def\FOnePathYF{1.1}   % R1
  
  % For R2 path
  \def\FTwoPathXA{1.0}  \def\FTwoPathYA{1.2}   % P0
  \def\FTwoPathXB{0.7}  \def\FTwoPathYB{1.0}
  \def\FTwoPathXC{0.3}  \def\FTwoPathYC{0.8}
  \def\FTwoPathXD{0.0}  \def\FTwoPathYD{0.8}
  \def\FTwoPathXE{-0.5} \def\FTwoPathYE{0.9}
  \def\FTwoPathXF{-0.9} \def\FTwoPathYF{1.4}   % R2
  
  % For R3 path
  \def\FThreePathXA{1.0}  \def\FThreePathYA{1.2}  % P0
  \def\FThreePathXB{0.9}  \def\FThreePathYB{1.5}
  \def\FThreePathXC{0.8}  \def\FThreePathYC{1.8}
  \def\FThreePathXD{0.85} \def\FThreePathYD{2.0}
  \def\FThreePathXE{0.9}  \def\FThreePathYE{2.2}
  \def\FThreePathXF{1.1}  \def\FThreePathYF{2.4}  % R3
  
  % For R4 path
  \def\FFourPathXA{1.0}  \def\FFourPathYA{1.2}   % P0
  \def\FFourPathXB{0.9}  \def\FFourPathYB{0.9}
  \def\FFourPathXC{0.8}  \def\FFourPathYC{0.6}
  \def\FFourPathXD{0.65} \def\FFourPathYD{0.35}
  \def\FFourPathXE{0.5}  \def\FFourPathYE{0.1}
  \def\FFourPathXF{0.1}  \def\FFourPathYF{-0.05} % R4

  % Forward path gradient descent-like approximations (dashed with arrows)
  % For R1 - Gradient descent zigzag approximation
  \draw[->, dashed, brightorange, opacity=0.8, very thick] 
    (\FOnePathXA,\FOnePathYA) -- 
    ({\FOnePathXB+0.1},{\FOnePathYB-0.1}) -- 
    ({\FOnePathXB+0.1},{\FOnePathYB+0.1}) -- 
    ({\FOnePathXC-0.1},{\FOnePathYC-0.1}) -- 
    ({\FOnePathXC+0.1},{\FOnePathYC+0.1}) -- 
    ({\FOnePathXD-0.1},{\FOnePathYD-0.1}) -- 
    ({\FOnePathXD+0.1},{\FOnePathYD+0.1}) -- 
    ({\FOnePathXE-0.1},{\FOnePathYE-0.1}) -- 
    ({\FOnePathXE+0.1},{\FOnePathYE+0.1}) -- 
    (\FOnePathXF,\FOnePathYF);

  % For R2 - Gradient descent zigzag approximation
  \draw[->, dashed, brightorange, opacity=0.8, very thick] 
    (\FTwoPathXA,\FTwoPathYA) -- 
    ({\FTwoPathXB-0.1},{\FTwoPathYB-0.1}) -- 
    ({\FTwoPathXB-0.3},{\FTwoPathYB+0.3}) -- 
    ({\FTwoPathXC+0.1},{\FTwoPathYC-0.1}) -- 
    ({\FTwoPathXC-0.1},{\FTwoPathYC+0.1}) -- 
    ({\FTwoPathXD+0.1},{\FTwoPathYD-0.1}) -- 
    ({\FTwoPathXD-0.1},{\FTwoPathYD+0.1}) -- 
    ({\FTwoPathXE+0.7},{\FTwoPathYE-0.7}) -- 
    ({\FTwoPathXE-0.1},{\FTwoPathYE+0.1}) -- 
    (\FTwoPathXF,\FTwoPathYF);
    
  % For R3 - Gradient descent zigzag approximation
  \draw[->, dashed, brightorange, opacity=0.8, very thick] 
    (\FThreePathXA,\FThreePathYA) -- 
    ({\FThreePathXB+0.1},{\FThreePathYB-0.1}) -- 
    ({\FThreePathXB-0.1},{\FThreePathYB+0.1}) -- 
    ({\FThreePathXC+0.4},{\FThreePathYC-0.4}) -- 
    ({\FThreePathXC-0.1},{\FThreePathYC+0.1}) -- 
    ({\FThreePathXD+0.1},{\FThreePathYD-0.1}) -- 
    ({\FThreePathXD-0.1},{\FThreePathYD+0.1}) -- 
    ({\FThreePathXE+0.6},{\FThreePathYE-0.6}) -- 
    ({\FThreePathXE-0.1},{\FThreePathYE+0.1}) -- 
    (\FThreePathXF,\FThreePathYF);
  
  % For R4 - Gradient descent zigzag approximation
  \draw[->, dashed, brightorange, opacity=0.8, very thick] 
    (\FFourPathXA,\FFourPathYA) -- 
    ({\FFourPathXB-0.1},{\FFourPathYB-0.1}) -- 
    ({\FFourPathXB+0.1},{\FFourPathYB-0.1}) -- 
    ({\FFourPathXC-0.4},{\FFourPathYC-0.4}) -- 
    ({\FFourPathXC+0.1},{\FFourPathYC-0.1}) -- 
    ({\FFourPathXD-0.6},{\FFourPathYD-0.6}) -- 
    ({\FFourPathXD+0.1},{\FFourPathYD-0.1}) -- 
    ({\FFourPathXE-0.1},{\FFourPathYE-0.1}) -- 
    ({\FFourPathXE+0.1},{\FFourPathYE-0.1}) -- 
    (\FFourPathXF,\FFourPathYF);
  
  % Draw the backward paths (solid with arrows)
  % Continuous versions
  \draw[->, very thick, brightpurple] (R1) .. controls (2.3,1.5) and (1.7,1.5) .. (P0);
  \draw[->, very thick, brightpurple] (R2) .. controls (-0.4,1.6) and (0.3,1.5) .. (P0);
  \draw[->, very thick, brightpurple] (R3) .. controls (1.3,1.9) and (1.2,1.6) .. (P0);
  \draw[->, very thick, brightpurple] (R4) .. controls (0.5,0.5) and (0.7,0.8) .. (P0);
  
  % Backward Monte Carlo dotted paths - with simplified Brownian motion-like behavior
  % For R1
  \foreach \i in {1,...,8} {
    % Random starting point near R1
    \pgfmathsetmacro{\startX}{2.9+0.1*rnd-0.05}
    \pgfmathsetmacro{\startY}{1.1+0.1*rnd-0.05}
    
    % Create path with multiple segments to simulate Brownian motion
    \draw[->, dotted, brightolive, ultra thick, opacity=0.9] 
      (\startX,\startY)
      % Point 1
      -- ++(0.1*rnd-0.05, 0.025*rnd*\i-0.05) 
      -- ++(0.1*rnd-0.05, -0.1-0.01*rnd*\i+0.05)
      -- ++(0.1*rnd-0.05, -0.15+0.1*rnd*\i+0.05)
      -- ++(-0.3-0.1*rnd+0.05, -0.1-0.1*rnd+0.05)
      -- ++(-0.4+0.1*rnd*\i+0.05, 0.2*rnd-0.05)
      -- ++(-0.5-0.1*rnd+0.05, 0.1*rnd-0.05)
      -- (P0);
  }
  
  % For R2
  \foreach \i in {1,...,8} {
    % Random starting point near R2
    \pgfmathsetmacro{\startX}{-0.9+0.1*rnd-0.05}
    \pgfmathsetmacro{\startY}{1.4+0.1*rnd-0.05}
    
    % Create path with multiple segments to simulate Brownian motion
    \draw[->, dotted, brightolive, ultra thick, opacity=0.9] 
      (P0)
      -- ++(-0.1*rnd-0.05, 0.1*rnd-0.05) 
      -- ++(-0.3+0.1*rnd-0.05, 0.001*rnd*\i-0.05)
      -- ++(-0.4+0.1*rnd*\i-0.05, 0.1-0.01*rnd*\i+0.05)
      -- ++(-0.3+0.01*rnd*\i-0.05, 0.1-0.01*rnd*\i+0.05)
      -- ++(-0.4+0.0025*rnd*\i-0.05, 0.1-0.05*rnd*\i+0.05)
      -- ++(-0.3+0.1*rnd*\i-0.05, 0.1*rnd*\i-0.05)
      -- (\startX, \startY);
  }
  
  % For R3
  \foreach \i in {1,...,8} {
    % Random starting point near R3
    \pgfmathsetmacro{\startX}{1.2+0.06*rnd*\i-0.05}
    \pgfmathsetmacro{\startY}{2.4+0.1*rnd-0.05}
    
    % Create path with multiple segments to simulate Brownian motion
    \draw[->, dotted, brightolive, ultra thick, opacity=0.9] 
     (P0)
      -- ++(0.025*\i*rnd-0.05, 0.2-0.1*rnd+0.05) 
      -- ++(-0.1*rnd-0.05, 0.3-0.1*rnd+0.05)
      -- ++(0.1+0.05*\i*rnd+0.05, 0.2-0.1*rnd+0.05)
      -- ++(0.1-0.1*rnd+0.05, 0.2-0.1*rnd+0.05)
      -- ++(-0.1*rnd-0.05, 0.2-0.1*rnd+0.05)
      -- ++(-0.1*rnd-0.05, 0.1-0.1*rnd+0.05)
      --  (\startX,\startY);
  }
  
  % For R4
  \foreach \i in {1,...,8} {
    % Random starting point near R4
    \pgfmathsetmacro{\startX}{0.1+0.1*rnd-0.05}
    \pgfmathsetmacro{\startY}{-0.05+0.1*rnd-0.05}
    
    % Create path with multiple segments to simulate Brownian motion
    \draw[->, dotted, brightolive, ultra thick, opacity=0.9] 
      (\startX,\startY)
      -- ++(0.1*rnd-0.05, 0.1*rnd-0.05) 
      -- ++(0.1+0.1*rnd-0.05, 0.2+0.1*rnd-0.05)
      -- ++(0.1+0.1*rnd-0.05, 0.3+0.1*rnd-0.05)
      -- ++(0.1+0.1*rnd-0.05, 0.2+0.1*rnd-0.05)
      -- ++(0.2+0.1*rnd-0.05, 0.2+0.1*rnd-0.05)
      -- ++(0.1+0.1*rnd-0.05, 0.1+0.1*rnd-0.05)
      -- (P0);
  }
  
  % Mark the reward points with labels
  \foreach \point/\lbl/\pos/\xshift/\yshift in {
    R1/R_1/right/0.3/0,
    R2/R_2/left/-0.3/0,
    R3/R_3/above/0/0.3,
    R4/R_4/below/0/-0.3
  } {
    \fill[rewardcolor] (\point) circle (0.06);
    \node[\pos] at ($({\point}) + ({\xshift},{\yshift})$) {\footnotesize $\lbl$};
  }
  
  % Mark P_0 with a star
  \node[star, star points=5, star point ratio=2.5, draw, fill=yellow, inner sep=0pt, minimum size=0.15cm] at (P0) {};

  
  % Mark P_0
  \fill[black] (P0) circle (0.05);
  \node[right] at (P0) {$P_0$};
  

  % Legend
  \node[anchor=north west, align=left, font=\small] at (5,3) {
    \textbf{Legend:}\\
    \textcolor{brightblue}{$\longrightarrow$} Forward paths\\
    \textcolor{brightorange}{$\dashrightarrow$} Forward gradient descent approx.\\
    \textcolor{brightpurple}{$\longrightarrow$} Backward paths\\
    \textcolor{brightolive}{$\cdot\cdot\cdot\cdot\rightarrow$} Backward Monte Carlo samples\\
    \textcolor{rewardcolor}{$\bullet$} Reward points\\
    \textcolor{yellow}{$\bigstar$} Starting point $P_0$
  };

\end{tikzpicture}

==> sparse-reward-figure.tex <==
\begin{tikzpicture}[scale=1.5]
    % Define gradient colors
    \definecolor{lowcolor}{RGB}{240,240,240}
    \definecolor{highcolor}{RGB}{70,130,180}
    % Define colors
    \definecolor{darkblue}{RGB}{0,0,150}
    \definecolor{brightblue}{RGB}{0,80,255}
    \definecolor{brightpurple}{RGB}{180,0,180}
    \definecolor{brightorange}{RGB}{255,120,0}
    \definecolor{brightorange}{RGB}{255,140,0}
    \definecolor{brightolive}{RGB}{120,160,0}
    
    
    % Define the non-convex shape with a smooth boundary
    \def\nonconvexshape{
      % Main blob shape
      (0,0) .. controls (1.5,0.5) and (2.5,-0.5) .. 
      (3,1) .. controls (3.5,2.5) and (2,3) .. 
      (1,2.5) .. controls (0.5,2.7) and (-0.5,2.2) .. 
      (-1,1.5) .. controls (-1.2,0.5) and (-0.8,-0.5) .. 
      (0,0) -- cycle
    }
    
    % Define reward points (sparse non-zero function values on/near boundary)
    \coordinate (R1) at (2.9,1.1);  % Reward point 1
    \coordinate (R2) at (-0.9,1.4); % Reward point 2
    \coordinate (R3) at (1.1,2.4);  % Reward point 3
    \coordinate (R4) at (0.1,-0.05); % Reward point 4
    
    % Define center point P_0
    \coordinate (P0) at (1.0,1.2);
    
    % Draw the base shape with gradient coloring
    \fill[lowcolor] \nonconvexshape;
    
    % Create radial fading gradients from each reward point
    \begin{scope}
      \clip \nonconvexshape;
      \foreach \point/\rad/\opac in {
        R1/1.2/0.8,
        R2/1.0/0.7,
        R3/1.1/0.9,
        R4/0.9/0.6
      } {
        \shade[inner color=highcolor, outer color=lowcolor, opacity=\opac] 
          (\point) circle (\rad);
      }
    \end{scope}
    
    % Draw the shape outline
    \draw[thick] \nonconvexshape;
    
    % Draw the forward paths (solid with arrows)
    % Continuous versions
    \draw[->, very thick, brightblue] (P0) .. controls (1.8,1.0) and (2.6,0.8) .. (R1);
    \draw[->, very thick, brightblue] (P0) .. controls (0.3,0.8) and (-0.5,0.9) .. (R2);
    \draw[->, very thick, brightblue] (P0) .. controls (0.8,1.8) and (0.9,2.2) .. (R3);
    \draw[->, very thick, brightblue] (P0) .. controls (0.8,0.6) and (0.5,0.1) .. (R4);
    
    % Extract the coordinates along the continuous forward paths
    % For R1 path
    \def\FOnePathXA{1.0}  \def\FOnePathYA{1.2}   % P0
    \def\FOnePathXB{1.3}  \def\FOnePathYB{1.15}
    \def\FOnePathXC{1.8}  \def\FOnePathYC{1.0}
    \def\FOnePathXD{2.2}  \def\FOnePathYD{0.9}
    \def\FOnePathXE{2.6}  \def\FOnePathYE{0.8}
    \def\FOnePathXF{2.9}  \def\FOnePathYF{1.1}   % R1
    
    % For R2 path
    \def\FTwoPathXA{1.0}  \def\FTwoPathYA{1.2}   % P0
    \def\FTwoPathXB{0.7}  \def\FTwoPathYB{1.0}
    \def\FTwoPathXC{0.3}  \def\FTwoPathYC{0.8}
    \def\FTwoPathXD{0.0}  \def\FTwoPathYD{0.8}
    \def\FTwoPathXE{-0.5} \def\FTwoPathYE{0.9}
    \def\FTwoPathXF{-0.9} \def\FTwoPathYF{1.4}   % R2
    
    % For R3 path
    \def\FThreePathXA{1.0}  \def\FThreePathYA{1.2}  % P0
    \def\FThreePathXB{0.9}  \def\FThreePathYB{1.5}
    \def\FThreePathXC{0.8}  \def\FThreePathYC{1.8}
    \def\FThreePathXD{0.85} \def\FThreePathYD{2.0}
    \def\FThreePathXE{0.9}  \def\FThreePathYE{2.2}
    \def\FThreePathXF{1.1}  \def\FThreePathYF{2.4}  % R3
    
    % For R4 path
    \def\FFourPathXA{1.0}  \def\FFourPathYA{1.2}   % P0
    \def\FFourPathXB{0.9}  \def\FFourPathYB{0.9}
    \def\FFourPathXC{0.8}  \def\FFourPathYC{0.6}
    \def\FFourPathXD{0.65} \def\FFourPathYD{0.35}
    \def\FFourPathXE{0.5}  \def\FFourPathYE{0.1}
    \def\FFourPathXF{0.1}  \def\FFourPathYF{-0.05} % R4
  
    % Forward path gradient descent-like approximations (dashed with arrows)
    % For R1 - Gradient descent zigzag approximation
    \draw[->, dashed, brightorange, opacity=0.8, very thick] 
      (\FOnePathXA,\FOnePathYA) -- 
      ({\FOnePathXB+0.1},{\FOnePathYB-0.1}) -- 
      ({\FOnePathXB+0.1},{\FOnePathYB+0.1}) -- 
      ({\FOnePathXC-0.1},{\FOnePathYC-0.1}) -- 
      ({\FOnePathXC+0.1},{\FOnePathYC+0.1}) -- 
      ({\FOnePathXD-0.1},{\FOnePathYD-0.1}) -- 
      ({\FOnePathXD+0.1},{\FOnePathYD+0.1}) -- 
      ({\FOnePathXE-0.1},{\FOnePathYE-0.1}) -- 
      ({\FOnePathXE+0.1},{\FOnePathYE+0.1}) -- 
      (\FOnePathXF,\FOnePathYF);
  
    % For R2 - Gradient descent zigzag approximation
    \draw[->, dashed, brightorange, opacity=0.8, very thick] 
      (\FTwoPathXA,\FTwoPathYA) -- 
      ({\FTwoPathXB-0.1},{\FTwoPathYB-0.1}) -- 
      ({\FTwoPathXB-0.1},{\FTwoPathYB+0.1}) -- 
      ({\FTwoPathXC+0.1},{\FTwoPathYC-0.1}) -- 
      ({\FTwoPathXC-0.1},{\FTwoPathYC+0.1}) -- 
      ({\FTwoPathXD+0.1},{\FTwoPathYD-0.1}) -- 
      ({\FTwoPathXD-0.1},{\FTwoPathYD+0.1}) -- 
      ({\FTwoPathXE+0.1},{\FTwoPathYE-0.1}) -- 
      ({\FTwoPathXE-0.1},{\FTwoPathYE+0.1}) -- 
      (\FTwoPathXF,\FTwoPathYF);
      
    % For R3 - Gradient descent zigzag approximation
    \draw[->, dashed, brightorange, opacity=0.8, very thick] 
      (\FThreePathXA,\FThreePathYA) -- 
      ({\FThreePathXB+0.1},{\FThreePathYB-0.1}) -- 
      ({\FThreePathXB-0.1},{\FThreePathYB+0.1}) -- 
      ({\FThreePathXC+0.1},{\FThreePathYC-0.1}) -- 
      ({\FThreePathXC-0.1},{\FThreePathYC+0.1}) -- 
      ({\FThreePathXD+0.1},{\FThreePathYD-0.1}) -- 
      ({\FThreePathXD-0.1},{\FThreePathYD+0.1}) -- 
      ({\FThreePathXE+0.1},{\FThreePathYE-0.1}) -- 
      ({\FThreePathXE-0.1},{\FThreePathYE+0.1}) -- 
      (\FThreePathXF,\FThreePathYF);
    
    % For R4 - Gradient descent zigzag approximation
    \draw[->, dashed, brightorange, opacity=0.8, very thick] 
      (\FFourPathXA,\FFourPathYA) -- 
      ({\FFourPathXB-0.1},{\FFourPathYB-0.1}) -- 
      ({\FFourPathXB+0.1},{\FFourPathYB-0.1}) -- 
      ({\FFourPathXC-0.1},{\FFourPathYC-0.1}) -- 
      ({\FFourPathXC+0.1},{\FFourPathYC-0.1}) -- 
      ({\FFourPathXD-0.1},{\FFourPathYD-0.1}) -- 
      ({\FFourPathXD+0.1},{\FFourPathYD-0.1}) -- 
      ({\FFourPathXE-0.1},{\FFourPathYE-0.1}) -- 
      ({\FFourPathXE+0.1},{\FFourPathYE-0.1}) -- 
      (\FFourPathXF,\FFourPathYF);
    
    % Draw the backward paths (solid with arrows)
    % Continuous versions
    \draw[->, very thick, brightpurple] (R1) .. controls (2.3,1.5) and (1.7,1.5) .. (P0);
    \draw[->, very thick, brightpurple] (R2) .. controls (-0.4,1.6) and (0.3,1.5) .. (P0);
    \draw[->, very thick, brightpurple] (R3) .. controls (1.3,1.9) and (1.2,1.6) .. (P0);
    \draw[->, very thick, brightpurple] (R4) .. controls (0.5,0.5) and (0.7,0.8) .. (P0);
    
    % Backward Monte Carlo dotted paths - with simplified Brownian motion-like behavior
    % For R1
    \foreach \i in {1,...,8} {
      % Random starting point near R1
      \pgfmathsetmacro{\startX}{2.9+0.1*rnd-0.05}
      \pgfmathsetmacro{\startY}{1.1+0.1*rnd-0.05}
      
      % Create path with multiple segments to simulate Brownian motion following the continuous path
      \draw[->, dotted, brightolive, thick, opacity=0.7] 
        (\startX,\startY)
        % Follow curve similar to the continuous path R1 to P0
        -- ++(0.05*rnd-0.025, 0.15+0.05*rnd-0.025) 
        -- ++(-0.15-0.05*rnd+0.025, 0.1+0.05*rnd-0.025)
        -- ++(-0.25-0.05*rnd+0.025, 0.05*rnd-0.025)
        -- ++(-0.3-0.05*rnd+0.025, -0.05-0.05*rnd+0.025)
        -- ++(-0.4-0.05*rnd+0.025, -0.1-0.05*rnd+0.025)
        -- ++(-0.5-0.05*rnd+0.025, -0.05-0.05*rnd+0.025)
        -- (P0);
    }
    % For R2
    \foreach \i in {1,...,8} {
      % Random starting point near R2
      \pgfmathsetmacro{\startX}{-0.9+0.1*rnd-0.05}
      \pgfmathsetmacro{\startY}{1.4+0.1*rnd-0.05}
      
      % Create path with multiple segments to simulate Brownian motion following the purple path
      \draw[->, dotted, brightolive, thick, opacity=0.7] 
        (\startX,\startY)
        -- ++(0.15+0.1*rnd-0.05, 0.15+0.1*rnd-0.05) 
        -- ++(0.25+0.1*rnd-0.05, 0.05+0.1*rnd-0.05)
        -- ++(0.3+0.1*rnd-0.05, -0.05-0.1*rnd+0.05)
        -- ++(0.35+0.1*rnd-0.05, -0.15-0.1*rnd+0.05)
        -- ++(0.3+0.1*rnd-0.05, -0.1-0.1*rnd+0.05)
        -- ++(0.25+0.1*rnd-0.05, -0.05+0.1*rnd-0.05)
        -- (P0);
    }
    
    % For R3
    \foreach \i in {1,...,8} {
      % Random starting point near R3
      \pgfmathsetmacro{\startX}{1.1+0.1*rnd-0.05}
      \pgfmathsetmacro{\startY}{2.4+0.1*rnd-0.05}
      
      % Create path with multiple segments to simulate Brownian motion following the purple path
      \draw[->, dotted, brightolive, thick, opacity=0.7] 
        (\startX,\startY)
        -- ++(0.1*rnd-0.05, -0.2-0.1*rnd+0.05) 
        -- ++(0.05*rnd-0.025, -0.25-0.05*rnd+0.025)
        -- ++(-0.05-0.05*rnd+0.025, -0.2-0.05*rnd+0.025)
        -- ++(-0.1-0.05*rnd+0.025, -0.15-0.05*rnd+0.025)
        -- ++(-0.05-0.05*rnd+0.025, -0.1-0.05*rnd+0.025)
        -- ++(0.05*rnd-0.025, -0.1-0.05*rnd+0.025)
        -- (P0);
    }
    % For R4
    \foreach \i in {1,...,8} {
      % Random starting point near R4
      \pgfmathsetmacro{\startX}{0.1+0.1*rnd-0.05}
      \pgfmathsetmacro{\startY}{-0.05+0.1*rnd-0.05}
      
      % Create path with multiple segments to simulate Brownian motion following the purple path
      \draw[->, dotted, brightolive, thick, opacity=0.7] 
        (\startX,\startY)
        -- ++(0.15+0.1*rnd-0.05, 0.2+0.1*rnd-0.05) 
        -- ++(0.2+0.1*rnd-0.05, 0.25+0.1*rnd-0.05)
        -- ++(0.25+0.1*rnd-0.05, 0.2+0.1*rnd-0.05)
        -- ++(0.15+0.1*rnd-0.05, 0.15+0.1*rnd-0.05)
        -- ++(0.1+0.1*rnd-0.05, 0.2+0.1*rnd-0.05)
        -- ++(0.05+0.1*rnd-0.05, 0.1+0.1*rnd-0.05)
        -- (P0);
    }
    % Mark the reward points with labels
    \foreach \point/\lbl/\pos/\xshift/\yshift in {
      R1/R_1/right/0.3/0,
      R2/R_2/left/-0.3/0,
      R3/R_3/above/0/0.3,
      R4/R_4/below/0/-0.3
    } {
      \fill[black] (\point) circle (0.06);
      \node[\pos] at ($({\point}) + ({\xshift},{\yshift})$) {\footnotesize $\lbl$};
    }
    
    % Mark P_0 with a star
    \node[star, star points=5, star point ratio=2.5, draw, fill=yellow, inner sep=0pt, minimum size=0.4cm] at (P0) {};
  
    
    % Mark P_0
    %\fill[black] (P0) circle (0.05);
    %\node[right] at (P0) {$P_0$};
    
  
    % Legend
    \node[anchor=north west, align=left, font=\small] at (4,3) {
      \textbf{Legend:}\\
      \textcolor{brightblue}{$\longrightarrow$} Forward paths\\
      \textcolor{brightorange}{$--\!\!\!-\!\!\!-\!\!\!\!\rightarrow$} Forward gradient descent approx.\\
      \textcolor{brightpurple}{$\longrightarrow$} Backward paths\\
      \textcolor{brightolive}{$\cdot\cdot\cdot\cdot\rightarrow$} Backward Monte Carlo samples\\
      \textcolor{black}{$\bullet$} Reward points\\
      \textcolor{yellow}{$\bigstar$} Starting point $P_0$
    };
  
  \end{tikzpicture}
